Unpaired Depth Super-Resolution in the Wild

Depth maps captured with commodity sensors are often of low quality and resolution; these maps need to be enhanced to be used in many applications. State-of-the-art data-driven methods of depth map super-resolution rely on registered pairs of low- and high-resolution depth maps of the same scenes. Acquisition of real-world paired data requires specialized setups. Another alternative, generating low-resolution maps from high-resolution maps by subsampling, adding noise and other artificial degradation methods, does not fully capture the characteristics of real-world low-resolution images. As a consequence, supervised learning methods trained on such artificial paired data may not perform well on real-world low-resolution inputs. We consider an approach to depth super-resolution based on learning from unpaired data. While many techniques for unpaired image-to-image translation have been proposed, most fail to deliver effective hole-filling or reconstruct accurate surfaces using depth maps. We propose an unpaired learning method for depth super-resolution, which is based on a learnable degradation model, enhancement component and surface normal estimates as features to produce more accurate depth maps. We propose a benchmark for unpaired depth SR and demonstrate that our method outperforms existing unpaired methods and performs on par with paired.

==> [DELETE] OLD files/bak.04.1-datasets.tex <==
\subsection{Datasets}
\label{experiments:datasets}

\OV{}% Предлагаемая структура раздела
% Нашей целью было собрать бенчмарк с такими-то характеристиками / с помощью которого можно было бы делать то-то.
We created a benchmark to compare both paired and unpaired methods for depth enhancement and super-resolution.
To that end we need a training data suitable for training both paired and unpaired methods on the same terms.
And we need a common test set which consists of RGB-D data from depth sensor and corresponding high quality depth of resolution of RGB image.

Our benchmark includes two training and one testing dataset.
Each dataset consists of three sets of RGB-D images:
source set~$\src$ with low-quality, low-resolution depth maps,
target set~$\tgt$ with high-quality, high-resolution depth maps,
and the set~$\tgtdown$ with the same high-quality depth maps as in the set~$\tgt$
but downsampled to the resolution of the set~$\src$.

% Для этого мы использовали датасеты ScanNet и InteriorNet.
% ScanNet представляет из себя то-то (что по сути, размер, характеристики изображений).
% InteriorNet представляет из себя то-то.
% На основе датасетов ScanNet и InteriorNet мы подготовили три части нашего бенчмарка.
As a sources of datasets to create our benchmark we selected ScanNet~\cite{ScanNet:Dai2017} which contains RGB-D from Structure depth sensor\footnote{\url{structure.io}} and InteriorNet~\cite{InteriorNet:Li2018} as a source oh high-quality RGB-D data from a simulator.ScanNet~\cite{ScanNet:Dai2017} contains RGB-D images captured with Structure depth sensor with $640 \times 480$ depth maps and $1280 \times 960$ color images. ScanNet data is used as $\tgtdown$~set during test and one of the training setups. To get the high-resolution $1280 \times 960$ depth maps for the set~$\tgtdown$ we rendered the 3D models of the ScanNet scenes,
reconstructed with BundleFusion~\cite{BundleFusion:Dai2017}. We refer to that dataset as \textbf{RenderScanNet} dataset.
In comparison to the raw depth maps, the depth values in these renderings are defined almost everywhere, and the noise is reduced by depth fusion.

% Первая часть, которую мы назвали ScanNet-RenderScanNet, представляет из себя то-то (что по сути, размер, характеристики изображений).
% (Сюда же можно встроить предложение из текущего текста
% "Each dataset consists of three sets of RGB-D images ... but downsampled to the resolution of the set~$\src$.")
% Она нужна для того чтобы то-то.
Our benchmark has two training setups for unpaired methods: 1) when \textbf{RenderScanNet} dataset is a source of high-quality data set~$\tgt$, and 2) when synthetic InteriorNet~\cite{InteriorNet:Li2018} dataset is used as set~$\tgt$. While source set~$\src$ of low-resolution and low-quality data is always data from ScanNet. The former setup is referred to as \textbf{ScanNet-RenderScanNet}. The latter setup we call as \textbf{ScanNet-InteriorNet}.
This setup helps to additionally evaluate unpaired methods in real-life usecase of training with synthetic data as a source of $\tgt$ set of high-quality data. This scenario is more complex for training, since sythetic scenes are different from real-world scenes in more aspects (like type of objects, depth range distribution) than renders from \textbf{RenderScanNet}.

% (Здесь можно сказать, почему мы оставили для обучения патчи а не целые изображения.)
% Вторая часть, которую мы назвали ScanNet-InteriorNet, представляет из себя то-то (что по сути, размер, характеристики изображений).
For paired methods we have only \textbf{ScanNet-RenderScanNet} training setup, since for such approaches we need RGB-D data from sensor as set~$\src$ and corresponding high-quality and high-resolution depth data as set~$\tgt$. Such paired data we have only for that case, while for InteriorNet~\cite{InteriorNet:Li2018} dataset we do not have any corresponding RGB-D data from depth sensor.
% Она нужна для того чтобы то-то.
% Третья часть, которую мы назвали Testing dataset, представляет из себя то-то (что по сути, размер, характеристики изображений).
% Она нужна для того чтобы то-то.
The \textbf{Testing dataset} of our benchmark consists of pairs from ScanNet and \textbf{RenderScanNet}.
To build the \textbf{Testing dataset} we manually selected 501 whole images
corresponding to the crops with no misalignment and with the distribution of hole sizes similar to the raw ScanNet.
This was necessary for a more accurate evaluation of the ability of methods to fill in missing values.

% Для получения хай-рез таргетов в датасетах ScanNet-RenderScanNet и Testing dataset мы использовали стратегию (похожую на?) [11].
% Конкретно, мы сделали фьюжен и отрендерили меши на камеры из датасета.
% Т.к есть мизалайнмент и артефакты фьюжена, мы дополнительно обработали пары чтобы оставить только хорошие.
% Для этого мы разрезали изображения на патчи такого-то размера (какого?) так-то (как?)
% и посчитали между патчами SSIM --- [ссылка] и что это такое в двух словах.
The first training dataset \textbf{ScanNet-RenderScanNet} is based on ScanNet~\cite{ScanNet:Dai2017},
which contains RGB-D images captured with Structure depth sensor
with $640 \times 480$ depth maps and $1280 \times 960$ color images.
We used these images to build the set~$\src$, as we describe below.
To get the high-resolution $1280 \times 960$ depth maps for the set~$\tgtdown$ we rendered the 3D models of the ScanNet scenes, reconstructed with BundleFusion~\cite{BundleFusion:Dai2017}.
In comparison to the raw depth maps, the depth values in these renderings are defined almost everywhere,
and the noise is reduced by depth fusion.

To get high-quality depth maps paired with the low-quality depth maps and use the proposed evaluation framework,
we use the camera poses corresponding to the images from the set~$\src$ for rendering.
To filter out bad pairs, caused by misalignments of camera poses estimates w.r.t.~the 3D model,
we further obtained crops from the depth maps and followed a filtering strategy based on their structural similarity, as in~\cite{RecScanNet:Jeon2018}. We extracted 320$\times$320 crops from input RGB-D frames and corresponding  640$\times$640 crops from 2x renders. Then we measured structured similarity~\cite{SSIM:Zhou2004} (SSIM) between the raw depth crop and 2x downsampled version of render crop. And selected depth pairs with SSIM greater than 0.8, and discarding pairs if the rendering produces misaligned result relatively to the sensor depth.
finally, we applied additional post-processing described in the supplementary material.

% Для Testing dataset мы отобрали пары целых изображений, для которых бОльшая часть патчей (какая?) имела ССИМ выше порога (какого?),
% а затем вручную отобрали только лучшие пары изображений без мизалайнмента.
% Т.к процесс фильтрации изменил распределение данных в тестовой выборке относительно исходного датасета,
% мы дополнительно отсеяли изображения так, чтобы распределение missing values в тестовых изображениях соответствовало исходному.
To build the \textbf{Testing dataset} we manually selected 501 whole RGB-D frames from ScanNet and corresponding renders from \textbf{ScanNet-RenderScanNet} amongst those frames, where the number of crops with SSIM (between sensor depth and render depth) $\ge$ 0.8 were more than 8 (out of 12 total crops). We selected the crops with no misalignment and with the distribution of hole sizes (area of missing values) similar to the raw ScanNet. This was necessary for a more accurate evaluation of the ability of methods to fill in missing values.

% Для ScanNet-RenderScanNet TODO @OV
As described in Section~\ref{method:data}, we split the obtained crop pairs from train \textbf{RenderScanNet} in Train~\emph{A} and Train~\emph{B} parts.
We got 38,577 pairs in Train~\emph{A}, which we used to build the set~$\src$ for unsupervised methods.
However, since the filtering process described above retains only the low-quality crops with few missing values,
we used 6,221 whole low-quality depth maps corresponding to the crops with more realistic low-quality data. (SSIM will be low for the pairs when low-quality crop has many missing values). Therefore we selected 6221 full RGB-D frames from sensor from Train~\emph{A} and use them as set~$\src$ for unsupervised methods in our experiments.

We got 37,986 pairs in Train~\emph{B}, from which we built all three sets $\src,\tgt,\tgtdown$ for supervised methods,
and the high-quality parts of which we used to build the sets $\tgt,\tgtdown$ for unsupervised methods.

% Для ScanNet-InteriorNet TODO @OV
For the second training dataset \textbf{ScanNet-InteriorNet}
we built the low-quality source set~$\src$ from the whole sensor images from ScanNet,
and for the high-quality sets we used RGB-D images from InteriorNet~\cite{InteriorNet:Li2018}.
Note, that InteriorNet provides depth only in resolution $640 \times 480$, while RGB is $1280 \times 960$. Thus, we created 2x resolution depth maps, using pre-trained by ourselves SRFBN. That SRFBN was trained to do 2x SR on the \textbf{RenderScanNet} data. The pairs for training were 2x NN downsampled render and render $\tgt$. Since, InteriorNet depth is synthetic and therefore relatively high-quality, then the quality of artifitial 2x samples obtained by the approach discussed above, is also reasonably good.




Note, that for the three datasets (ScanNet, RenderScanNet, and InteriorNet), we select RGB-D frames with the maximum depth value not exceeding 5.1\,m, corresponding to the 85th depth range percentile in ScanNet~\cite{ScanNet:Dai2017}. 
Such filtering is consistent with the depth range where commercial depth sensors have sufficient precision. Meanwhile this simultaneously allows to reduce discrepancy better between images in synthetic and real datasets and providing common threshold for data normalization, which is a common practice for deep learning.

Combining ScanNet-RenderScanNet and Testing dataset allows to compare paired and unpaired methods on the common data,
while combining ScanNet-InteriorNet and Testing dataset allows to study the unpaired methods in a real-world unpaired learning scenario.

==> [DELETE] OLD files/bak.04.2-results.tex <==
\subsection{Experimental Results}
\label{experiments:results}
\OV{}% Предлагаемая структура
% Начинаем с того, что вообще мы делали в экспериментах и зачем, если можно как-то нетривиально ответить на вопрос "зачем". Т.е,
% Мы сравниваем наш метод в задаче 2х супер-рез глубины с парными и непарными методами.

% \DZ{it would be fine to start the results section with this}
In our experiments, we compare our approach for 2x depth super-resolution with paired and unpaired approaches.
For quantitative evaluation, we calculate pixel-wise metrics excluding the pixels without a definite ground truth value.
To measure the denoising and inpainting performance specifically,
we calculate $\text{RMSE}_d, \text{MAE}_d$ and $\text{RMSE}_h, \text{MAE}_h$,
taking into account only the pixels with definite low-quality depth values,
and only the pixels without the value, \ie., holes, respectively.
RMSE and MAE are in millimeters.



% Дополнительно, мы сравниваем в задаче enhancement. Подчеркиваем здесь, что enhancement на втором месте после супер-рез.
% Еще проводим ablation study чтобы ответить на такие-то вопросы (какие?).
Due to the design of our method (bicubic upsampling to technically increase spatial resolution), we also could use our method to perform depth enhancement with no change of depth resolution. Thus we provide additionally results on that tasks to show wide applicability of our method.


% Дальше уже описываем как именно мы проводили эксперименты.
% Всегда сначала мотивируем то что мы делаем, и только потом говорим, что мы делаем.
% В остальном, описание экспериментов нормальное, но не хватает конкретики по результатам,
% написано просто "наш метод лучше". А в чем конкретно лучше? можно ли написать, почему?


\noindent \textbf{Super-resolution.}
We consider the task of increasing a depth image resolution by a factor of two.
We compare our method with a state-of-the-art supervised method for depth super-resolution MS-PFL~\cite{MS-PFL:Chuhua2020}
and a method for RGB image super-resolution SRFBN~\cite{SRFBN:Li_2019}, applied to depth images.
Originally, these methods are trained on pairs of high-quality images and their downsampled versions.

% Из первой рецензии:
% "Why are the SOTA methods being re-trained for this paper's datasets?
% What limits usingthe datasets proposed in the SOTA papers to test the proposed model?
% I would like to understand the bias in theperformance due to the choice of the particular datasets in this paper." ---
% Надо как-то ненавязчиво подчеркнуть, что цель наших экспериментов --- сравнить методы в равных условиях,
% и поэтому мы не проводим эксперименты с датасетами из статей про СОТА методы.
The goal of our experiments to compare with other methods, especially paired ones, in the equal terms. Since the lack of the datasets to quantitatively evaulate performance on real sensor data, we trained investigated methods on our benchmark.

We trained them in two scenarios:
(1) on pairs from the sets $\src, \tgt$, \ie., with low-quality sensor data as the input,
and (2)  on pairs from the sets $\tgtdown, \tgt$, \ie., with the downsampled high-quality target as the input.
Since the input in the Testing dataset consists of low-quality sensor data,
the second scenario shows the performance in the wild of paired SR methods trained in a conventional way, on downsampled data.

To compare unsupervised methods with ours we combine them with upsampling.
Since image-to-image unsupervised methods applied to  depth maps produced relatively poor results for the enhancement task,
\ie., with the same image resolution of the input and output,
as we discuss further,
we report only the results produced by the enhancement method \cite{Gu2020_TIP} combined with upsampling.
We compare against several versions: 
(1) we train it on low-resolution depth maps from $\src, \tgtdown$,
and for testing upsample its output with bicubic interpolation
(denoted in tables as \textquote{\cite{Gu2020_TIP}+B}),
(2) or with SRFBN trained on pairs from $\tgtdown, \tgt$
(denoted as \textquote{\cite{Gu2020_TIP}+\cite{SRFBN:Li_2019}\textsuperscript{\textasteriskcentered}}),
or (3) train it on bicubically upsampled low-quality depth maps from $\src$ and high-resolution depth maps from $\tgt$,
and for testing apply it on top of bicubic interpolation
(\textquote{B+\cite{Gu2020_TIP}}).

The results on ScanNet-RenderScanNet in Table~\ref{tab:enh_and_sr_metrics} and Figure~\ref{fig:sr_render}
show that our method outperforms unsupervised methods and its performance is comparable to the supervised methods.
The results on ScanNet-InteriorNet in Table~\ref{tab:enh_and_sr_metrics_interior} and Figure~\ref{fig:sr_interior} show that our unpaired approach could perform well on real sensor depth while being trained with synthetic data as examples of $\tgt$ data.
% OV: If the results on both datasets show the above, then replace with
% The results on ScanNet-RenderScanNet in Table~\ref{tab:enh_and_sr_metrics} and Figure~\ref{fig:sr_render}
% and on ScanNet-InteriorNet in Table~\ref{tab:enh_and_sr_metrics_interior} and Figure~\ref{fig:sr_interior}
% show that our method outperforms unsupervised methods and is comparable to the supervised methods.


%------------------------------------------------------------------------

\noindent \textbf{Enhancement.}
We compare the version of our method that does not change image resolution, 
with a state-of-the-art unsupervised method for depth enhancement from Gu~\etal.~\cite{Gu2020_TIP},
as well as several RGB image translation methods:
CycleGAN~\cite{CycleGAN:Zhu2017},  U-GAT-IT~\cite{U-GAT-IT:Kim2020} and NiceGAN~\cite{NiceGAN:Chen2020}.
We trained these methods on either 1-channel depth maps, or, in case of CycleGAN, also on 4-channel RGB-D images.
We also compare our method with a state-of-the-art supervised method for depth enhancement LapDEN~\cite{RecScanNet:Jeon2018}.

Table~\ref{tab:enh_metrics} and Figure~\ref{fig:enh_render} show the results for the ScanNet-RenderScanNet datasets.
Our method successfully performs denoising and hole inpainting, and yields surface normals close to the target.
It produces fewer artefacts in comparison to all unsupervised methods and preserves the original depth range in contrast to them.
Quantitatively, our approach outperforms all unsupervised methods and is comparable to the supervised method.

We show some results on ScanNet-InteriorNet in Figure~\ref{fig:enh_interior} and refer to the supplementary materials for the additional visualizations and quantitative comparisons.


%------------------------------------------------------------------------

\noindent \textbf{Ablation study.}
%To validate advantages of our scheme we tested our building blocks. 

In our ablation study, networks are trained on \textbf{ScanNet-InteriorNet}. We trained our approach with several modifications in \emph{Translation Component} and \emph{Enhancement Component}. The results are shown in Table~\ref{tab:sr_ablation_int}. We demonstrate that to achieve low perceptual $\mathrm{MSE_v}$ we need use both generated pseudo-pairs and holes augmentation when training Enhancement Component~$\openh$. Further, with our \emph{Translation Component} the method yields better results compared to using CycleGANs. An ablation study of the enhancement version of our method on \textbf{ScanNet-InteriorNet} can be found in the supplementary document.

%------------------------------------------------------------------------

%We evaluate our method on both depth enhancement and 2x depth super-resolution.
%Real sensor depth is noisy and has many missing values, and in both tasks method is required to produce higher quality depth, without missing values and noise. But for SR the additional requirement is to produce output of higher resolution. Note, that for SR, we first apply Bicubic upsampling to depth, and then apply our Enhancement Component. Thus we could use our method for both depth SR and enhancement.

% \DZ{The introductory sentences talking about SR and enhancement in a way that puts othese on equal footing I would drop this }
% Since our method is capable of both super-resolution and 1-to-1 enhancement, with the same image resolution of the input and output, we evaluate it on both of these tasks.

% We experimentally found that pre-traing our method for 1-to-1 enhancement before training it for super-resolution leads to improved results.
% \OV{what specifically? better/faster convergence, results of higher quality}
% \OV{commented out because it does not belong here, this is implementation}
% \DZ{too much enhancement too little super-resolution -- I'd also vote for dropping this}
% We show that our method with unpaired training of the Enhancement Component performs on par with paired methods designed for depth maps,
% outperforms image-to-image translation methods adapted for depth maps,
% and outperforms the unpaired depth enhancement method by Gu~\cite{Gu2020_TIP}.
% \OV{Maybe this sentence should be in the intro?}


==> src/figures/fig_enhancement_training.tex <==

\begin{figure}[t]
    \centerline{\includegraphics[width=\linewidth]{our_scheme.pdf}}
    \caption{Training scheme for the Enhancement Component.}
    \label{fig:fig_enhancement_training}
\end{figure}


==> src/main/figures.tex <==
\newpage
\break
\afterpage{

\clearpage
}


==> src/note_sup.tex <==
\begin{table*}[]
    \centerline{
    \begin{threeparttable}
    \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & RMSE $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & MAE $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$ \\ \hline
        Gu \textit{et~al.}~\cite{Gu2020_TIP} & 107.30 & 290.05 & 66.75 & 46.12 & 200.97 & 33.10 & 0.4441\\ \hline
        Ours & 80.75 & 208.51 & 59.77 & 34.65 & 150.73 & 25.99 & 0.1906\\ \hline \midrule
    \end{tabular}
%
    % \begin{tablenotes}
    %   \small
    %   \item \textasteriskcentered - Depth as input \\
    %   \textdagger - Depth concatenated with RGB as input
    % \end{tablenotes}
    \end{threeparttable}
    }
    \caption{The enhancement results ScanNet~\cite{InteriorNet:Li2018}-InteriorNet~\cite{InteriorNet:Li2018}}
    \label{tab:enh_metrics_interior}
\end{table*}

\begin{table*}[]
    \centerline{
    \begin{threeparttable}
    \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & RMSE $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & MAE $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$ \\ \hline
        Bicubic & 14.25 & 31.127 & 11.78 & 1.36 & 5.29 & 1.12 & 0.04\\
        $\text{SRFBN}$~\cite{SRFBN:Li_2019} & 6.55 & 15.16 & 5.00 & 0.61 & 1.20 & 0.57 & 0.09\\
        $\text{MS-PFL}$~\cite{MS-PFL:Chuhua2020} & 15.81 & 35.67 & 12.36 & 4.46 & 9.09 & 4.05 & 0.11\\ \hline \midrule
    \end{tabular}
%
    % \begin{tablenotes}
    %   \small
    %   \item
    % \end{tablenotes}
    \end{threeparttable}
    }
    \caption{The results for SR of the reproduction using the original code,
    and of our experiments.}
    \label{tab:naive_sr_metrics}
\end{table*}

\begin{table*}[]
    \centerline{
    \begin{threeparttable}
    \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & RMSE $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & MAE $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$ \\ \hline
        With CycleGAN~\cite{CycleGAN:Zhu2017} translation & 86.98 & 208.41 & 67.22 & 43.47 & 158.58 & 34.47 & 0.1727\\
        Without Img2Depth & 98.90 & 298.70 & 58.67 & 34.33 & 224.22 & 20.25 & 0.1638\\
        Only Img2Depth & 277.39 & 331.19 & 271.59 & 227.02 & 274.61 & 223.32 & 0.4486\\ \hline
        Ours & 77.07  & 169.55 & 63.31 & 32.99 & 110.06 & 27.26 & 0.1194 \\ \hline \midrule
    \end{tabular}
%
    % \begin{tablenotes}
    %   \small
    %   \item
    % \end{tablenotes}
    \end{threeparttable}
    }
    \caption{ Ablation}
    \label{tab:ablation}
\end{table*}
%http://tug.ctan.org/info/symbols/comprehensive/symbols-a4.pdf
\subsection{Datasets}
We used two collections of depth data: the first one, low-quality: with low resolution and natural shortcomings(noise and missing values). And the second one, high-quality: with high resolution, noise and holes-free. We rendered ScanNet~\cite{ScanNet:Dai2017} meshes for every 50th pose and used these reconstructed depth frames as a second high-quality dataset - RenderScanNet with resolution $1280 \times 960$.

In all three datasets, we selected such frames for which the maximum depth value doesn't exceed 5.1 meters, which is the 85th percentile in the ScanNet~\cite{ScanNet:Dai2017}. Such filtering is consistent with the depth range, in which commercial depth sensors have sufficient precision, allows better matching between synthetic and real datasets, and provides a natural way for data normalization, which is a common practice for Deep Learning.
The rendering process can produce local misalignments, as shown in~\cite{RecScanNet:Jeon2018}, and creates unnatural regions in high-quality data. To breakdown this problem we filtered rendered depth, similar to~\cite{RecScanNet:Jeon2018}. We sliced frames into 320$\times$320 and 640$\times$640 patches and measured the structured similarity (SSIM) between the raw and corresponding downsampled rendered depth patch. We filtered out such pairs that have SSIM lower than 0.8, also we discarded pairs if the rendering fails to fill in missing values.

\subsection{Results}

First of all, we measure the effectiveness of a depth enhancement at low resolution.
% , since this is a prerequisite for obtaining a satisfactory high resolution, as shown in Fig.~\ref{fig:sr_fails}.
For comparison, we chose the unsupervised image-to-image translation method CycleGAN~\cite{CycleGAN:Zhu2017} and two recent methods: U-GAT-IT~\cite{U-GAT-IT:Kim2020}, NiceGAN~\cite{NiceGAN:Chen2020}. The main method for comparison is SOTA unsupervised method for depth enhancement Gu \textit{et~al.}~\cite{Gu2020_TIP} and as a reference, we compared with SOTA supervised method for depth enhancement LapDEN~\cite{RecScanNet:Jeon2018}. The refine depth frame is shown in Fig.~\ref{fig:enh_render}.
% This example shows that all methods are more or less capable of filling holes and quantitative comparison better shows the quality of holes inpainting. 
The quality of denoising, as well as artifacts created by methods, is better seen on surface normals, and visual comparison shows, that the proposed method successfully performs denoising and creates smooth surface normals close to $\text{render}_{1x}$ and to result of supervised method LapDEN~\cite{RecScanNet:Jeon2018}; produces much fewer artifacts, in comparison with all unsupervised methods; preserves original depth range after transformation, with which some unsupervised methods fail. The quality of holes inpainting better to compare on quantitative metrics. Our approach outperforms all unsupervised methods and is comparable to the supervised method, which is confirmed quantitatively in Table~\ref{tab:enh_metrics}. 
% The results of the metrics within the regions of missing values of our method are closest to the result obtained using the supervised method, which may indicate that the proposed model performs semantically meaningful filling of holes, and not simply filling with average values. Good denoising quality is confirmed by low $\text{MSE}_v$ value, which are designed to highlight it~\cite{PDSR:Voynov2019}.
All methods was trained on ScanNet~\cite{ScanNet:Dai2017}-RenderScanNet datasets, metrics was evaluated on ($\text{raw}_{1X}$, $\text{render}_{1X}$) pairs from test scenes.

We also showed that our approach could be trained on unpaired dataset which consists of ScanNet~\cite{ScanNet:Dai2017} and InteriorNet~\cite{InteriorNet:Li2018}. The visual example for all methods, except supervised, on Fig.~\ref{fig:enh_interior} and quantitatively comparison in Table~\ref{tab:enh_metrics_interior}. These results show that our approach also outperforms the related methods in such a scenario.

==> src/sup/05.2-results.tex <==
\section{Experimental Results}
\label{supp:sec:results}

Following our evaluation framework, we compare depth SR methods trained on pairs $(\tgtdown, \tgt)$ of \mbox{RGB-D} images and tested on $\tgt$ from the held-out test set. 
Quantitative comparison in Table~\ref{tab:naive_sr} suggests that SRFBN~\cite{SRFBN:Li_2019} performs favourably to both simple Bicubic upsampling and MS-PFL method~\cite{MS-PFL:Chuhua2020}; we thus used SRFBN as an upsampling operation to get high-resolution synthetic frames from InteriorNet. 

We provide more qualitative enhancement results for the \textbf{ScanNet-RenderScanNet} scenario in Figure~\ref{fig:sup_enh_scannet_rscannet}; results for the \textbf{ScanNet-InteriorNet} scenario are presented in Table~\ref{tab:sup_enh_interior} and Fig.~\ref{fig:sup_enh_scannet_interiornet}.


More qualitative results on SR task for \textbf{ScanNet-RenderScanNet} scenario are shown in Fig.~\ref{fig:sup_sr_scannet_rscannet} and for \textbf{ScanNet-InteriorNet} scenario in Fig.~\ref{fig:sup_sr_scannet_interiornet}.


\begin{table}[]
    \centerline{
    \resizebox{.99\columnwidth}{!}{
    \begin{threeparttable}
    \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & RMSE $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & MAE $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$ \\ \hline
        Bicubic & \underline{14.25} & \underline{31.127} & \underline{11.78} & \underline{1.36} & \underline{5.29} & \underline{1.12} & \textbf{0.04}\\
        $\text{SRFBN}$~\cite{SRFBN:Li_2019} & \textbf{6.55} & \textbf{15.16} & \textbf{5.00} & \textbf{0.61} & \textbf{1.20} & \textbf{0.57} & \underline{0.09}\\
        $\text{MS-PFL}$~\cite{MS-PFL:Chuhua2020} & 15.81 & 35.67 & 12.36 & 4.46 & 9.09 & 4.05 & 0.11\\ \hline \midrule
    \end{tabular}
    \end{threeparttable}
    }
    }
    \caption{SR results for methods trained on $(\tgtdown, \tgt)$ applied to $\tgtdown$. The best result is in bold, the second best is underlined.}
    \label{tab:naive_sr}
\end{table}

\begin{table}
    \centerline{
    \resizebox{.99\columnwidth}{!}{
    \begin{threeparttable}
    % \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength{\tabcolsep}{0.2\tabcolsep}% Shrink \tabcolsep by 30%
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & $\text{RMSE}$ $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & $\text{MAE}$ $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$  \\ \hline
        $\text{UDSR}$\tnote{\textbullet} \xspace  & 86.98 &  \underline{208.41} & 67.22 & \underline{158.58} & 43.47 & 34.47 & 0.1727\\
        $\text{UDSR}$\tnote{\textdagger} \xspace & 98.90 &  298.70 & \textbf{58.67} & 224.22 & 34.32 & \textbf{20.25} & \underline{0.1638}\\
        $\fimg$ & 277.38 & 331.19 & 271.59 & 274.61 & 227.01 & 223.32 & 0.4486\\ \hline
        UDSR  & 77.07 & \textbf{169.55} & \underline{63.31} &  \textbf{110.06} & \textbf{32.99} & \underline{27.26} & \textbf{0.1194} \\ \hline \midrule
    \end{tabular}
    \begin{tablenotes}
    \footnotesize
        \item[\textbullet] - our model with replacement translation model by CycleGAN~\cite{CycleGAN:Zhu2017}
        \item[\textdagger]  - our model without $\fimg$
    \end{tablenotes}
    \end{threeparttable}
    }
    }
    \caption{ Enhancement ablation on \textbf{ScanNet-RenderScanNet} scenario.}
    \label{tab:enh_ablation_scan}
\end{table}

\begin{table}
    \centerline{
    \resizebox{.99\columnwidth}{!}{
    \begin{threeparttable}
    \setlength{\tabcolsep}{0.2\tabcolsep}% Shrink \tabcolsep by 30%
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & $\text{RMSE}$ $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & $\text{MAE}$ $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$  \\ \hline
        $\text{UDSR}$\tnote{\textbullet} \xspace  & 163.73 &  206.95 & 157.97 & 143.52 & 157.10 & 142.31 & 0.2549\\
        $\text{UDSR}$\tnote{$\ddagger$} \xspace & \underline{74.40}  & \underline{167.08}   & \underline{58.82}   & \underline{27.18}   & \underline{101.18}   & \underline{21.11}   & \textbf{0.1338}\\
        $\text{UDSR}$\tnote{$\ast$} \xspace & 85.48 & 218.16   & 61.09   & 32.03   & 137.16 & 23.53 & 0.1786 \\
        $\text{UDSR}$\tnote{$\star$} \xspace  & 75.97 & 171.38 & 59.48 & 27.84  & 102.69   & 21.55 & \underline{0.1430} \\ \hline
        $\text{UDSR}$\tnote{\textdagger} \xspace  & 93.49 &  256.92 & 61.42 & 35.65 & 171.48 & 25.13 & 0.2044\\
        $\text{UDSR}$\tnote{\textsection} \xspace & 85.48  & 218.16  & 61.09  & 32.03 & 137.16 & 23.53 & 0.1786 \\
        $\text{UDSR}$\tnote{$\diamond$} \xspace  & 92.08 & 257.50 & \textbf{57.98} & 31.28  & 194.32  & \textbf{18.45} & 0.1432 \\
        $\text{UDSR}$\tnote{$\circ$} \xspace  & \textbf{72.98} & \textbf{158.98} & 59.16 & \textbf{26.65}  & \textbf{92.36}   & 21.36 & 0.2063\\ \hline
        UDSR   & 80.83 & 199.88 & 59.12 & 29.92 & 124.78 & 22.18 & 0.1467\\ \hline \midrule
    \end{tabular}
    \begin{tablenotes}
    \footnotesize
        \item[\textbullet] Ours with translation network $\GenTgtSrc$ replaced by CycleGAN~\cite{CycleGAN:Zhu2017}
        \item[$\ddagger$] Ours with translation network $\GenTgtSrc$ trained without surface normal discriminators $\discNmapTgt, \discNmapSrc$ 
        \item[$\ast$] Ours with translation network $\GenTgtSrc$ trained without $\text{MSE}_\text{v}$ loss 
        \item[$\star$] Ours with translation network trained without depth range loss
        \item[\textdagger] Ours without $\fimg$
        \item[\textsection] Ours without any surface normal term loss in Enhancement network
        \item[$\diamond$] Ours with enhancement network $\fenh$ trained without additional holes
        \item[$\circ$] Ours with enhancement network $\fenh$ trained without pseudo examples
        % \item[$\ast$] Ours with translation network $\GenTgtSrc$ trained without $\text{MSE}_\text{v}$ loss in cycle consistency term and without surface normal discriminators $\discNmapTgt, \discNmapSrc$
    \end{tablenotes}
    \end{threeparttable}
    }
    }
    \caption{Enhncement ablation on \textbf{ScanNet-InteriorNet} scenario.}
    \label{tab:enh_ablation_int}
\end{table}

\begin{table}
    \centerline{
    \resizebox{.99\columnwidth}{!}{% <------ Don't forget this %
    \begin{threeparttable}
    \setlength{\tabcolsep}{0.2\tabcolsep}% Shrink \tabcolsep by 30%
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & $\text{RMSE}$ $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & $\text{MAE}$ $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$  \\ \hline
        $\text{UDSR}$\tnote{\textbullet} \xspace & 208.86   & 238.39 & 203.81 & 188.47   & 183.73 & 188.18 & 0.3934 \\
        $\text{UDSR}$\tnote{$\ddagger$} \xspace & 88.18   & 213.28 & 66.05 & 38.56   & 135.22 & 31.01 & 0.2442\\
        $\text{UDSR}$\tnote{$\ast$} \xspace & 89.29   & 208.58 & 69.28 & 43.42  & 135.04 & 36.27 & \underline{0.2361} \\
        $\text{UDSR}$\tnote{$\star$} \xspace  & 81.49   & \underline{192.00} & 63.08 & 32.25   & \underline{119.43} & 25.44 & \textbf{ 0.2299} \\ \hline
        $\text{UDSR}$\tnote{\textdagger} \xspace & 117.43   & 376.28 & 66.53 & 45.01   & 271.50 & 29.73 & 0.4121 \\
        $\text{UDSR}$\tnote{\textsection} \xspace & 94.06   & 228.43 & 71.56 & 44.75  & 151.09 & 36.64 & 0.3512 \\
        $\text{UDSR}$\tnote{$\diamond$} \xspace & 110.41   & 342.05 & 66.17 & 45.25   & 279.85 & 28.83 & 0.2875 \\
        $\text{UDSR}$\tnote{$\circ$} \xspace  & \textbf{78.07}   & \textbf{177.67} & \underline{62.75} & \underline{30.25}   & \textbf{104.18} & \underline{24.59} & 0.4315 \\ \hline
        UDSR  & \underline{81.12}  & 197.86 & \textbf{60.95} & \textbf{27.97}   & 123.50 & \textbf{20.59} & 0.2605  \\ \hline \midrule
        % $\text{UDSR}$\tnote{$\ast$} \xspace & \underline{180.92} & 66.09 & \underline{111.25} & 30.98 & \underline{0.2396} \\
    \end{tabular}
    \begin{tablenotes}
    \footnotesize
        \item[\textbullet] Ours with translation network $\GenTgtSrc$ replaced by CycleGAN~\cite{CycleGAN:Zhu2017}
        \item[$\ddagger$] Ours with translation network $\GenTgtSrc$ trained without surface normal discriminators $\discNmapTgt, \discNmapSrc$ 
        \item[$\ast$] Ours with translation network $\GenTgtSrc$ trained without $\text{MSE}_\text{v}$ loss 
        \item[$\star$] Ours with translation network trained without depth range loss
        \item[\textdagger] Ours without $\fimg$
        \item[\textsection] Ours without any surface normal term loss in Enhancement network
        \item[$\diamond$] Ours with enhancement network $\fenh$ trained without additional holes
        \item[$\circ$] Ours with enhancement network $\fenh$ trained without pseudo examples
        % \item[$\ast$] Ours with translation network $\GenTgtSrc$ trained without $\text{MSE}_\text{v}$ loss in cycle consistency term and without surface normal discriminators $\discNmapTgt, \discNmapSrc$
    \end{tablenotes}
    \end{threeparttable}
    }
    }
    \caption{Ablation of SR on \textbf{ScanNet-InteriorNet}.}
    \label{tab:sr_ablation_int}
\end{table}


% First of all, we measured the effectiveness of a depth enhancement.
% , since this is a prerequisite for obtaining a satisfactory high resolution, as shown in Fig.~\ref{fig:sr_fails}.
We compare the effectiveness of our method on unpaired depth enhancement, comparing to three image-based methods: CycleGAN~\cite{CycleGAN:Zhu2017}, U-GAT-IT~\cite{U-GAT-IT:Kim2020}, and NiceGAN~\cite{NiceGAN:Chen2020}. 
The closest to our enhancement approach method is unsupervised depth enhancement method by Gu \textit{et~al.}~\cite{Gu2020_TIP}.
% Unlikewe further provide results by a supervised method for depth enhancement LapDEN~\cite{RecScanNet:Jeon2018} as a reference.
All methods were trained on ScanNet-InteriorNet datasets, metrics were evaluated on ($\src$, $\tgtdown$) pairs from test scenes.

% We present the depth frames resulting from all methods in Figures~\ref{fig:sup_enh_scannet_rscannet}--\ref{fig:sup_enh_scannet_interiornet}.
% This example shows that all methods are more or less capable of filling holes and quantitative comparison better shows the quality of holes inpainting. 
Improvements in denoising performance are most notable when observing surface normals. 
In this respect, our proposed method produces smooth surfaces that are close to the renderings $\tgtdown$; in comparison with all unsupervised methods, we produce much fewer surface and depth artifacts. We also better preserve original depth range after transformation, while other unsupervised methods may suffer from distortions.
% Overall, our approach performs on par with the supervised LapDEN~\cite{RecScanNet:Jeon2018}.

Considering hole inpainting, our approach again outperforms all unsupervised methods and is comparable to the supervised method, according to $\text{RMSE}_d$ and $\text{MAE}_d$, see Table~\ref{tab:sup_enh_interior}.
% The results of the metrics within the regions of missing values of our method are closest to the result obtained using the supervised method, which may indicate that the proposed model performs semantically meaningful filling of holes, and not simply filling with average values. Good denoising quality is confirmed by low $\text{MSE}_v$ value, which are designed to highlight it~\cite{PDSR:Voynov2019}.

Our approach is additionally validated by training on the unpaired dataset which consists of ScanNet and InteriorNet.
The visual comparison is provided in Fig.~\ref{fig:sup_enh_scannet_interiornet} and Fig.~\ref{fig:sup_sr_scannet_interiornet}; quantitative comparison in Table~\ref{tab:sup_enh_interior}.
These results show that our approach also outperforms competitor methods in such a scenario and could produce results close to depth fusion approach \cite{BundleFusion:Dai2017} being trained on synthetic InteriorNet dataset as instances of high-quality depth. 

\iffalse
    \begin{figure*}
        % \vspace{-1.5em}
            \begin{tikzpicture}
                \node[inner sep=0] (image) {\includegraphics[width=.95\linewidth]{img/sup_sr_int_abl.pdf}};
                \begin{scope}[shift=(image.north west), x={(image.north east)},y={(image.south west)}]
                    \node at (.05, -.04) {\footnotesize {Input ($\src$)}};
                    \node at (.15, -.04) {\footnotesize {$\text{UDSR}^{\bullet}$}};
                    \node at (.23, -.04) {\footnotesize {$\text{UDSR}^\ddagger$}};
                    \node at (.32, -.04) {\footnotesize {$\text{UDSR}^\ast$}};
                    \node at (.41, -.04) {\footnotesize {$\text{UDSR}^\star$}};
                    \node at (.50, -.04) {\footnotesize {$\text{UDSR}^\dagger$}};
                    \node at (.59, -.04) {\footnotesize {$\text{UDSR}^\S$}};
                    \node at (.68, -.04) {\footnotesize {$\text{UDSR}^\diamond$}};
                    \node at (.77, -.04) {\footnotesize {$\text{UDSR}^\circ$}};
                    \node at (.86, -.04) {\footnotesize {UDSR}};
                    \node at (.955, -.04) {\footnotesize {Reference ($\tgt$)}};
                \end{scope}
        	\end{tikzpicture}
        \caption{Ablation of SR on \textbf{ScanNet-InteriorNet}. Same notation as in Table~\ref{tab:sr_ablation_int}.}
    	\label{fig:sup_sr_ablation_int}
    \end{figure*}
    
    \begin{figure*}
        % \vspace{-1.5em}
            \begin{tikzpicture}
                \node[inner sep=0] (image) {\includegraphics[width=.95\linewidth]{img/sup_enh_int_abl.pdf}};
                \begin{scope}[shift=(image.north west), x={(image.north east)},y={(image.south west)}]
                    \node at (.05, -.04) {\footnotesize {Input ($\src$)}};
                    \node at (.15, -.04) {\footnotesize {$\text{UDSR}^{\bullet}$}};
                    \node at (.23, -.04) {\footnotesize {$\text{UDSR}^\ddagger$}};
                    \node at (.32, -.04) {\footnotesize {$\text{UDSR}^\ast$}};
                    \node at (.41, -.04) {\footnotesize {$\text{UDSR}^\star$}};
                    \node at (.50, -.04) {\footnotesize {$\text{UDSR}^\dagger$}};
                    \node at (.59, -.04) {\footnotesize {$\text{UDSR}^\S$}};
                    \node at (.68, -.04) {\footnotesize {$\text{UDSR}^\diamond$}};
                    \node at (.77, -.04) {\footnotesize {$\text{UDSR}^\circ$}};
                    \node at (.86, -.04) {\footnotesize {UDSR}};
                    \node at (.955, -.04) {\footnotesize {Reference ($\tgt$)}};
                \end{scope}
        	\end{tikzpicture}
        \caption{Ablation of Enhancement on \textbf{ScanNet-InteriorNet}. Same notation as in Table~\ref{tab:enh_ablation_int}.}
    	\label{fig:enh_ablation_int}
    \end{figure*}
    
    \begin{figure*}
        % \vspace{-1.5em}
        \begin{center}
            \begin{tikzpicture}
                \node[inner sep=0] (image) {\includegraphics[width=0.95\textwidth,height=0.95\textheight,keepaspectratio]{img/s_enhancement_render.pdf}};
                \begin{scope}[shift=(image.north west), x={(image.north east)},y={(image.south west)}]
                \node at (.06, -.01) {\footnotesize {Input ($\src$)}};
                \node at (.17, -.01) {\footnotesize {$\text{CycleGAN}^{\text{\textbullet}}$}};
                \node at (.28, -.01) {\footnotesize {$\text{CycleGAN}^{\text{\textdagger}}$}};
                \node at (.39, -.01) {\footnotesize {$\text{U-GAT-IT}$}};
                \node at (.50, -.01) {\footnotesize {$\text{NiceGAN}$}};
                \node at (.61, -.01) {\footnotesize {Gu}};
                \node at (.72, -.01) {\footnotesize {LapDEN}};
                \node at (.83, -.01) {\footnotesize {Ours}};
                \node at (.94, -.01) {\footnotesize {Reference ($\tgt$)}};
                \end{scope}
            \end{tikzpicture}
        \end{center}
        \caption{Qualitative depth enhancement results for the \textbf{ScanNet-RenderScanNet} scenario.}
        \label{fig:sup_enh_scannet_rscannet}
    \end{figure*}
    
    \begin{figure*}
        % \vspace{-1.5em}
        \begin{center}
            \begin{tikzpicture}
                \node[inner sep=0] (image) {\includegraphics[width=0.95\textwidth,height=0.95\textheight,keepaspectratio]{img/s_enhancement_interior.pdf}};
                \begin{scope}[shift=(image.north west), x={(image.north east)},y={(image.south west)}]
                \node at (.06, -.01) {\footnotesize {Input ($\src$)}};
                \node at (.19, -.01) {\footnotesize {$\text{CycleGAN}^{\text{\textbullet}}$}};
                \node at (.31, -.01) {\footnotesize {$\text{CycleGAN}^{\text{\textdagger}}$}};
                \node at (.43, -.01) {\footnotesize {$\text{NiceGAN}$}};
                \node at (.56, -.01) {\footnotesize {$\text{U-GAT-IT}$}};
                \node at (.68, -.01) {\footnotesize {Gu}};
                \node at (.81, -.01) {\footnotesize {Ours}};
                \node at (.94, -.01) {\footnotesize {Reference ($\tgt$)}};
                \end{scope}
            \end{tikzpicture}
        \end{center}
        \caption{Qualitative depth enhancement results for \textbf{ScanNet-InteriorNet} scenario.}
        \label{fig:sup_enh_scannet_interiornet}
    \end{figure*}
    \begin{figure*}
        % \vspace{-1.5em}
        \begin{center}
            \begin{tikzpicture}
                \node[inner sep=0] (image) {\includegraphics[width=0.95\textwidth,height=0.95\textheight,keepaspectratio]{img/s_sr_render.pdf}};
                \begin{scope}[shift=(image.north west), x={(image.north east)},y={(image.south west)}]
                \node at (.06, -.01) {\footnotesize {Input ($\src$)}};
                \node at (.16, -.01) {\footnotesize {$\text{SRFBN}^\text{\textsection}$}};
                \node at (.26, -.01) {\footnotesize {$\text{MS-PFL}^{\text{\textsection}}$}};
                \node at (.36, -.01) {\footnotesize {$\text{SRFBN}^\text{\textasteriskcentered}$}};
                \node at (.45, -.01) {\footnotesize {$\text{MS-PFL}^{\text{\textasteriskcentered}}$}};
                \node at (.55, -.01) {\footnotesize {Gu+$\text{SRFBN}^\text{\textasteriskcentered}$}};
                \node at (.65, -.01) {\footnotesize {Gu+Bicubic}};
                \node at (.75, -.01) {\footnotesize {Bicubic+Gu}};
                \node at (.85, -.01) {\footnotesize {Ours}};
                \node at (.95, -.01) {\footnotesize {Reference ($\tgt$)}};
                \end{scope}
            \end{tikzpicture}
        \end{center}
        \caption{Qualitative results for depth SR for \textbf{ScanNet-RenderScanNet} scenario.}
        \label{fig:sup_sr_scannet_rscannet}
    \end{figure*}
    
    \begin{figure*}
        % \vspace{-1.5em}
        \begin{center}
            \begin{tikzpicture}
                \node[inner sep=0] (image) {\includegraphics[width=0.95\textwidth,height=0.95\textheight,keepaspectratio]{img/s_sr_interior.pdf}};
                \begin{scope}[shift=(image.north west), x={(image.north east)},y={(image.south west)}]
                \node at (.08, -.01) {\footnotesize {Input ($\src$)}};
                \node at (.27, -.01) {\footnotesize {Gu+$\text{SRFBN}^\text{\textasteriskcentered}$}};
                \node at (.42, -.01) {\footnotesize {Gu+Bicubic}};
                \node at (.59, -.01) {\footnotesize {Bicubic+Gu}};
                \node at (.75, -.01) {\footnotesize {Ours}};
                \node at (.92, -.01) {\footnotesize {Reference ($\tgt$)}};
                \end{scope}
            \end{tikzpicture}
        \end{center}
        \caption{Qualitative depth SR results for \textbf{ScanNet-InteriorNet} scenario.}
        \label{fig:sup_sr_scannet_interiornet}
    \end{figure*}
\else
\fi

==> src/sup/experiments_details.tex <==
% This is some details deleted from main text
% ========================================================
% \paragraph{Enhancement module.} 
% For $G_{enh}$ network, we also use a standard U-Net. To improve  inpainting performance, for each RGBD frame on each iteration with probability 0.9, we randomly added $N$ rectangular holes, with 
% $N$ uniformly sampled in 10 to 60 range.
% The holes have random sizes ($h_n$, $w_n$) where $h_n$ is uniformly sampled from $H/128\ldots H/8$, and $w_n$ from $W/128 \ldots W/8$  where H,W are the dimensions of he input depth image. 
% All weight  masks $w$ are described by two numbers: the weights of pixels with and without depth values.
% ========================================================

%For example $w^n_n$ = (1,2) means weight of pixels without holes = 1, weight of pixels with holes = 2.   

% ========================================================
% \paragraph{Rendered ScanNet.} 
% Firstly we used a batch size of 12. We trained $G_{enh}$ network 20k iterations with $lr$ equal to $1*10^{-3}$ and then train 40k iteration linearly reducing $lr$ to $4*10^{-4}$. As augmentation, we used random rotation, horizontal flip and random crops with size of $384 \times 512$. For detailed setup, we refer to the appendix.
% ========================================================

% We used followed weights: $\lambda_1^H$=15,  $w_{1d}^H$ = (1,30), $\lambda^H_2$=10, $w_{2d}^H$ = (0,20), $\lambda_{v2}^H$=2,  $w_{v2}^H$ = (1,5), $\lambda_{v1}^H=2$, $w_{v1}^H$ = (1,5), $\lambda_{TVR}^H=2*10^{-7}$, $\lambda_1^L$=40, $w_{1d}^L = (1,40)$,  $\lambda_2^L=20$, $w_{2d}^L$ = (0,20), $\lambda_{TVR}^L=2*10^{-7}$, $w_{edge}$ = 1.

% After that we drop learning rate to $2*10^{-4}$, turn off random crop, set batch size to 6. We trained scheme 10k iteration with new lr and then trained 20k iterations more evenly reducing lr to 0. Thus, overall we trained our $G_{enh}$ for 90k iterations. We also changed the following parameters: $w_{1d}^H$ = (1,100), $w_{2d}^H$ = (0,100), $\lambda_{v1}^H$=3,  $w_{1d}^L$ = (2,40), $w_{2d}^L$ = (0,50)). 

% For train SR we took our trained enhancement model and just fine-tune it for 5k iterations with learning rate $2*10^{-4}$ and then 15k iterations with evenly reducing learning rate to 0. In comparison with the previous set of parameters, we only changed the followed weight: $\lambda_{v2}^H$=3, $\lambda_{v1}^H$=3. For LQ pass input we use $\text{raw}_{2X}$ as input, for HQ pass input we use $\text{render}_{2X}$. Here we didn't use any augmentation.   

% ========================================================
% \paragraph{ScanNet-InteriorNet.}
% Firstly we used a batch size of 12. We trained $G_{enh}$ network 20k iterations with $lr=1*10^{-3}$ and then train 70k iterations linearly reducing $lr$ to 0. As augmentation, we used random rotation, horizontal flip and random crops with size of $384 \times 512$. For detailed setup, we refer to the supplementary materials.
% ========================================================


% We used followed weights: $\lambda_1^H$=10,  $w_{1d}^H$ = (1,30), $\lambda^H_2$=10, $w_{2d}^H$ = (0,10), $\lambda_{v2}^H$=3,  $w_{v2}^H$ = (1,5), $\lambda_{v1}^H$=2, $w_{v1}^H$ = (1,5), $\lambda_{TVR}^H$=$4*10^{-7}$, $\lambda_1^L$=40, $w_{1d}^L$ = (1,40),  $\lambda_2^L$=20, $w_{2d}^L$ = (0,25), $\lambda_{TVR}^L$=$4*10^{-7}$, $w_{edge}$ = 1.

% After that, we drop learning rate to $2*10^{-4}$, turn off random crop, set batch size to 6. We trained scheme 10k iteration with new learning rate and then trained 20k iterations more evenly reducing learning rate to 0. Thus, overall we trained our $G_{enh}$ for 120k iterations.

% For train SR we took our trained enhancement model and just fine-tune it for 5k iterations with learning rate $2*10^{-4}$ and then 15k iterations with evenly reducing learning rate to 0. As augmentation, we use random crop with size (384, 512), random rotation, and horizontal flip. After that we turn off all augmentation set learning rate $1*10^{-4}$
% train 5k iterations and then 10k iterations with evenly reducing learning rate to 0
% In comparison with the previous set of parameters, we only changed the followed weights: $\lambda_{TVR}^H$=$2*10^{-7}$, $\lambda_{TVR}^L$=$2*10^{-7}$, $\lambda_1^L$=100.  



% \subsection{Implementation}
% In this section we cover some implementation details of our proposed UDSR \footnote{hidden for review; link will appear in camera-ready} 
% % \footnote{\url{github.com/keqpan/udsr}} 
% model. For more detailed setup we refer to supplementary materials.

% \noindent \textbf{Translation block.}
% Each generator takes RGB image and depth map and outputs depth. Image and depth features produced by the encoders are concatenated and processed by the ResNet blocks. Both generators have the same architecture and, at a high level, consist of separate feature extractors (encoders) for RGB images and depth maps, 9 ResNet blocks~\cite{ResNet:He2015}, and a decoder. Finally, the decoder outputs depth map. Discriminators have the same architecture as in the original CycleGan~\cite{CycleGAN:Zhu2017}, however, we use Spectral Normalization~\cite{SpectralNorm:Miyato2018} for weights regularization. Thus we do not use any feature normalization in discriminators.

% \noindent \textbf{Enhancement module.}
% Image guidance network $\text{G}_{I}$ consists of two parts: image feature extractor, and main part (depth-prediction network) that compute depth predictions. The feature extractor includes 2 downsampling blocks,  6 ResNet blocks, 2 upsampling blocks. The depth-prediction network is a standard U-Net. We use Instance Normalization \cite{DBLP:journals/corr/UlyanovVL16} in both parts. For $G_{enh}$ network, we also use a standard U-Net. 

\begin{table*}[]
    \centerline{
    \begin{threeparttable}
    \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & RMSE $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & MAE $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$ \\ \hline
        Bicubic & \underline{14.25} & \underline{31.127} & \underline{11.78} & \underline{1.36} & \underline{5.29} & \underline{1.12} & \textbf{0.04}\\
        $\text{SRFBN}$~\cite{SRFBN:Li_2019} & \textbf{6.55} & \textbf{15.16} & \textbf{5.00} & \textbf{0.61} & \textbf{1.20} & \textbf{0.57} & \underline{0.09}\\
        $\text{MS-PFL}$~\cite{MS-PFL:Chuhua2020} & 15.81 & 35.67 & 12.36 & 4.46 & 9.09 & 4.05 & 0.11\\ \hline \midrule
    \end{tabular}
    \end{threeparttable}
    }
    \caption{SR results for methods applied to $\text{render}_{1x}$. The best result is in bold, the second best is underlined.}
    \label{tab:naive_sr}
\end{table*}

%%%% ===== Tables added in re-submission. Moved here on Aug 18




\begin{table*}[]
    \centerline{
    \begin{threeparttable}
    \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Method & RMSE $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & MAE $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$ \\ \hline
        With CycleGAN~\cite{CycleGAN:Zhu2017} translation & \underline{86.98} & \underline{208.41} & 67.22 & 43.47 & \underline{158.58} & 34.47 & 0.1727\\
        Without $G_I$ & 98.90 & 298.70 & \textbf{58.67} & \underline{34.33} & 224.22 & \textbf{20.25} & \underline{0.1638} \\
        Only $G_I$ & 277.39 & 331.19 & 271.59 & 227.02 & 274.61 & 223.32 & 0.4486\\ \hline
        Ours & \textbf{77.07}  & \textbf{169.55} & \underline{63.31} & \textbf{32.99} & \textbf{110.06} & \underline{27.26} & \textbf{0.1194} \\ \hline \midrule
    \end{tabular}
    \end{threeparttable}
    }
    \caption{We provide more metrics for ablation study. The best result is in bold, the second best is underlined.}
\end{table*}


\begin{table*}
    \centerline{
    \begin{threeparttable}
    \setlength\tabcolsep{\widthof{0}*\real{.6}}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
         Method & RMSE $\downarrow$ & $\text{RMSE}_h$ $\downarrow$ & $\text{RMSE}_d$ $\downarrow$ & MAE $\downarrow$ & $\text{MAE}_h$ $\downarrow$ & $\text{MAE}_d$ $\downarrow$ & $\text{MSE}_v$ $\downarrow$ \\ \hline
        Gu \textit{et~al.}~\cite{Gu2020_TIP} + $\text{SRFBN}^{\text{\textasteriskcentered}}$\textsuperscript{\ref{note:graph}}~\cite{SRFBN:Li_2019} & 107.23 & 298.18 & \underline{67.81} & \underline{45.70} & 209.99 & \underline{33.12} & 0.4250\\
        Gu \textit{et~al.}~\cite{Gu2020_TIP} + Bicubic & \underline{107.14} & \underline{297.69} & 67.85 & 46.12 & \underline{209.92} & 33.57 & \underline{0.3670}\\
        Bicubic + Gu \textit{et~al.}~\cite{Gu2020_TIP} & 241.20 & 893.06 & 109.01 & 93.51 & 771.49 & 50.50 & 0.4794\\ 
        \hline
        UDSR(Ours) & \textbf{81.12} & \textbf{197.86} & \textbf{60.95} & \textbf{27.97} & \textbf{123.50} & \textbf{20.59} & \textbf{0.2605}\\ \hline \midrule
    \end{tabular}
%
    % \begin{tablenotes}
    %   \small
    %   \item
    % \end{tablenotes}
    \end{threeparttable}
    }
    \caption{The SR results for \textbf{ScanNet~\cite{ScanNet:Dai2017}-InteriorNet~\cite{InteriorNet:Li2018}} scenario.}
    \label{tab:enh_and_sr_metrics_interior}
\end{table*}

==> src/tables/tbl_arch_overview.tex <==
\begingroup
\renewcommand{\arraystretch}{1.15}
\begin{table}[h!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{p{2cm} p{5cm} p{2cm}}
\hline
Component & Training & Inference \\ \hline
Translation Component & Phase 1: Cycle-consistent unpaired training~$\to$ generate pseudo-examples (Section~\ref{method:translation}) & Not used \\ 
Enhancement Component & Phase 2: Supervised training with pseudo-examples (Section~\ref{method:enhancement}) & Direct \mbox{prediction} \\ \hline
\end{tabular}%
}
\caption{Component-wise view of our method.}
\label{tab:tbl_arch_overview}
\end{table}
\endgroup

